L2PF -- Learning to Prune Faster

Various applications in the field of autonomous driving are based on convolutional neural networks (CNNs), especially for processing camera data. The optimization of such CNNs is a major challenge in continuous development. Newly learned features must be brought into vehicles as quickly as possible, and as such, it is not feasible to spend redundant GPU hours during compression. In this context, we present Learning to Prune Faster which details a multi-task, try-and-learn method, discretely learning redundant filters of the CNN and a continuous action of how long the layers have to be fine-tuned. This allows us to significantly speed up the convergence process of learning how to find an embedded-friendly filter-wise pruned CNN. For ResNet20, we have achieved a compression ratio of 3.84 x with minimal accuracy degradation. Compared to the state-of-the-art pruning method, we reduced the GPU hours by 1.71 x.

==> cvip_rebuttal.tex <==
Response to CVIP 2020 reviewers 

Reviewer 1
Authors have proposed multi-task, try-andlearn method for CNN. After careful consideration of this paper. I found it shows a valid contributes to the field and well explained. I recommend the paper for inclusion in the conference.

Response 
Thank you for the positive response. 


Reviewer 2
This paper proposes a learning-based pruning algorithm to find the optimal number of finetuning epochs.


There are some grammatical errors in this paper. To mention a few,
1. In this context we present Learning to Prune Faster. (line #6- Abstract)
3. Xxxxxxxx to compress neurons, kernels or layers in xxxxxx (second paragraph, Page #2)
3. xxxx a RL framework can be xxxxx (first line, Section 3.1)

Although the reference to some important prior works is missing and the experiments are not enough, the reviewer still suggests accepting this paper. The author is expected to deal with the following concerns in the camera-ready version.

Response
Thank you for the valuable feedback. We have corrected the grammar errors in the revised version of the manuscript. 

1. He et al. [6] prune redundant filters based on the geometric mean heuristic of the filters. (in heuristic-based pruning techniques (Related work section))
However, this filter pruning method based on the geometric median.

Response: Thank you pointing out the error. We have chnaged it in the revised manuscript. 

2. Importantly, I feel the experimental part is weak since the authors have not conducted enough experiments. So, I suggest the authors to conduct experiments using VGG-16 over CIFAR-10 dataset to generalize the efficacy of the proposed method.

Response: Thank you for the suggestion.  In this work, the experiments are based on ResNet20 CNN model which is already an compressed baseline compared to VGG-16. In ResNet20, the number of filters in different convolutional layers could be either 16, 32 or 64. The number of filters in VGG-16 could be either 64, 128, 256 or 512. As VGG-16 is much more over-parameterized, there would be defineltly be more pruning scope. Due to the current time constraints for camera ready, we cannot train a VGG-16 baseline model and apply pruning using L2PF. 

3. Since the proposed method is a learning-based pruning technique, I recommend comparing the proposed method with the state-of-the-art (in Fig. 3) in terms of the overall time required.
Response: We have mentioned the number of fine-tune epochs which is measure of time needed for the pruning process. AMC, ALF require significantly less amount of overall time for pruning. As L2P and L2PF select filters not based on heuristics, every pruning strategy is evaluated after certain epochs of finetuning. In L2PF, the finetuning epochs are reduced using the continuous actions of RL-agent. 


4. I recommend to include one table for comparing the proposed learning-based filter pruning method with heuristic-based and In-train pruning methods.
Response: We have compared our method L2PF with other pruning methods in Fig. 3 detailing accuracy, compression ratio and pruning type. We have compared with AMC, L2P (learning based) and ALF (in-train). FPGM (heuristic based) also produced results on ResNet20 model but does not include number of parameters after pruning which is essential to report compression ratio. 

==> data/40_experiments/41_tabel_test.tex <==
\renewcommand{\arraystretch}{1.3}
\begin{table}[!h]
\centering
\caption[base model benchmarks]{Accuracy on validation, test dataset. and total number of parameters and Ops w/o FC}
  \label{tab:basemodel}
  \begin{tabular}{V{.2} V{.15} V{.15} V{.2} V{.14} V{.14}} 
  \toprule
    \textbf{Model} & \textbf{Accuracy valid} & \textbf{Accuracy test} &\textbf{Million Weights} & \textbf{Million Ops}\\
    \midrule
    ResNet18 \cite{he2015deep} & 92.0\% & 90.8\% & 0.26 & -\\
    \bottomrule
    %%\multicolumn{3}{l}{$^{1}$} \\
    \end{tabular}
\end{table}

==> misc/todoes.tex <==
\section*{ToDoes:}
\begin{todolist}
    \item Abstract
    \item Introduction
    \item Related Work
    \begin{todolist}
        \item Comparison table
        \item AMC
        \item Learning2Prune
        \item ChannelPruning
    \end{todolist}
    \item Multi-task learning
    \item Method
    \item Experiments
    \item Conclusion
    \item References
% \item[\done] Change Bibliograpystyle to splncs04
% \item Fix equations by using more mathmatical symbols, e.g. $\psi \leftarrow acc$,\\
% $\varphi^E \leftarrow Energy(Register,Input$
\end{todolist}
